Toward Self-Adjusting k-ary Search Tree Networks

Datacenter networks are becoming increasingly flexible with the incorporation of new networking technologies, such as optical circuit switches. These technologies allow for programmable network topologies that can be reconfigured to better serve network traffic, thus enabling a trade-off between the benefits (i.e., shorter routes) and costs of reconfigurations (i.e., overhead). Self-Adjusting Networks (SANs) aim at addressing this trade-off by exploiting patterns in network traffic, both when it is revealed piecewise (online dynamic topologies) or known in advance (offline static topologies). In this paper, we take the first steps toward Self-Adjusting k-ary tree networks. These are more powerful generalizations of existing binary search tree networks (like SplayNets), which have been at the core of SAN designs. k-ary search tree networks are a natural generalization offering nodes of higher degrees, reduced route lengths for a fixed number of nodes, and local routing in spite of reconfigurations. We first compute an offline (optimal) static network for arbitrary traffic patterns in $O(n^3 \cdot k)$ time via dynamic programming, and also improve the bound to $O(n^2 \cdot k)$ for the special case of uniformly distributed traffic. Then, we present a centroid-based topology of the network that can be used both in the offline static and the online setting. In the offline uniform-workload case, we construct this quasi-optimal network in linear time $O(n)$ and, finally, we present online self-adjusting k-ary search tree versions of SplayNet. We evaluate experimentally our new structure for $k=2$ (allowing for a comparison with existing SplayNets) on real and synthetic network traces. Our results show that this approach works better than SplayNet in most of the real network traces and in average to low locality synthetic traces, and is only little inferior to SplayNet in all remaining traces.

==> statements/arbitrary_workload_search_tree_theorem.tex <==
\begin{theorem}
    \label{thm:arbitrary wprkload}
	The problem to find a $k$-ary Search Tree with the minimal total distance can be solved in $O(n^3k^2)$.
\end{theorem}
\begin{proof}
Our algorithm uses the dynamic programming approach.
	
Throughout the proof, if we are talking about the segment $[i, j]$, we assume that $j \geq i$. 
	
We denote a submatrix of $D[i\ldots j, i\ldots j]$ as $D|_{[i, j]}$.
	
We define matrix $W \in \mathbb{N}_0^{n \times n}$:
	
\begin{align*}
	W[i, j] = \sum\limits_{u \in [n] \setminus [i,j]}\sum\limits_{v \in [i, j]}D[u, v] + D[v, u]
\end{align*}
Intuitively, this matrix shows a total number of requests going out of the segment $[i, j]$.
	
\input{paper/statements/precomputing_w_claim}

We define a cost of a segment $[i, j]$ as a cost of an optimal $k$-ary Search Tree build on that segment plus the number of requests going out of that segment.
\va{What this cost if giving us? The answer?}
\begin{align*}
	\mathrm{cost}(i, j) = \min\limits_{T}\mathrm{TotalDistance}(D|_{[i, j]}, T) + W[i, j]
\end{align*}

We finally define our dynamic for $1 \leq i \leq j \leq n$ and $1 \leq t \leq k$ as
	\begin{align*}
		dp[i][j][t] = \min\limits_{i = i_1 < i_2 < \ldots < i_{t + 1} = j + 1}\sum\limits_{p = 1}^tcost(i_{p}, i_{p + 1} - 1)
	\end{align*}
	
\va{How to calculate cost out of this dp?}
So $dp[i][j][t]$ intuitively means the minimal cost of partitioning a segment $[i, j]$ into $t$ children that are $k$-ary search trees.
    
\begin{align*}
    \begin{cases}
        dp[i][j][t] = \min\limits_{l \in [i, j - 1]}dp[i][l][1] + dp[l + 1][j][t - 1],\ t > 1\\
        dp[i][j][t] = \min\limits_{r \in [i, j]}\min\limits_{d_l + d_r \leq k} dp[i][r - 1][d_l] + dp[r + 1][j][d_r] + W[i, j],\ t = 1
    \end{cases}
\end{align*}

The logic is that in order to partition the segment into $t > 1$ trees one should first choose the prefix subsegment for the first tree and build $t - 1$ trees on the remaining segment. 
    
The case $t = 1$ is special. It means that we want to build a single search tree on the segment. In order to do so, we first choose the root node $r \in [i, j]$ and after that the number of children to the left of a root node $[i, r - 1]$ and a number of children to the right of a root node $[r + 1, j]$. This covers all the possible cases. And in each case we can minimize each subtree independently, so we just refer to the corresponding $dp$ value.

When calculating $d[i][j][t]$ we refer to the answer on subsegments of $[i, j]$, so we make sure that this value is already calculated by processing segments increasing their length. Namely, we start by setting the answer on the segments of length 1, and then proceed by considering all the segments of length 2, then 3 and so on up to $n$. 

So we need to consider all the possible segments, there are $O(n^2)$ of them. For each segment we calculate dynamic for $t \in [1, k]$. When $i, j$ and $t > 1$ are fixed, we spend $O(n)$ time iterating over $[i, j]$ looking for minimum, this results in $O(n^2(k - 1)n)$ in total. And when $i, j$ and $t = 1$ are fixed, we spend $O(n)$ considering different roots and $O(k^2)$ possibilities of distributing number of subtrees to the left and to the right to the root. So in this case we obtain $O(n^3k^2)$.  
\end{proof}

==> statements/cost_uniform_claim.tex <==
\begin{claim}
    \label{clm:cost uniform}
    In the uniform workload scenario, $cost(i, i  - 1 + l) = cost(j, j - 1 + l)$ for any $l \in [1, n]$ and any $i,j \in [1, n - l]$. In other words, cost of the segment depends only on its length, not position. 
\end{claim}
\begin{proof}
    Recall that 
    \begin{align*}
    	\mathrm{cost}(i, j) = \min\limits_{T}\mathrm{TotalDistance}(D|_{[i, j]}, T) + W[i, j]
    \end{align*}
    By the Claim \ref{clm:w uniform} the second term is equal for any two segments of an equal length. As for the first term, it is also equal since $D|_{[i, i - 1 + l]} = D|_{[j, j - 1 + l]}$ for all $i, j, l$ in the uniform case. 
\end{proof}

==> statements/edge_potential_sum.tex <==
\begin{claim}
	\begin{align*}
		\mathrm{TotalDistance}(D, T) = \sum\limits_{e \in E(T)}\mathrm{potential}(D, T, e)
	\end{align*}
\end{claim}

==> statements/flatten_theorem.tex <==
\begin{theorem}
	\label{thm:flatten}
	The difference in total distance between an optimal tree $T$ and the quasi-optimal tree is $O(n^2k\log(k))$.
\end{theorem}
\begin{proof}
	Our plan is to reconfigure $T$ into the quasi-optimal tree while controlling the total distance increase.
	
	We will push up the nodes to ensure that all the subtrees at level $l$ are weak-complete starting from $l = 2\lceil \log_2(9k) \rceil$ and up to $l = 0$ (the whole tree).
	
	So consider we want to make a subtree $S$ at level $l$ weak-complete. Since we go through levels decreasingly, we can argue that all the subtrees of $S$ are already weak-complete (this holds for $l = 2\lceil \log_2(9k) \rceil$).
	
	If $S$ is not weak-complete, it means that there are two subtrees of $S$ with height difference at least $2$. So we take the subtree with the biggest height and the subtree with the smallest height and perform a push up operation between them.
	
	We act so until there are two subtrees of height difference $\geq 2$. Once there are none, we say that $S$ is weak-complete by definition.
	
	When processing certain level, each node is moved at most once (in its subtree), so each node is moved no more then $2\lceil \log_2(9k) \rceil$ times, thus, by Corollary \ref{cor:push_up2} the total cost change is $O(n^2k\log(k))$.
\end{proof}

==> statements/lowerbound_theorem.tex <==
\begin{theorem}
	Assuming $k$ is a constant, the total distance in optimal tree $T$ is $\Omega(n^2\log(n))$
\end{theorem}
\begin{proof}
	At least two $T_i$s have $\geq \frac{n}{2k}$ nodes. Each such $T_i$ has $\Omega(n)$ nodes at levels $\geq \log_k(n) - 2$. Thus the distance between those nodes is $\Omega(n^2\log(n))$.
\end{proof}

==> statements/push_up_lemma.tex <==
\begin{lemma}
	\label{lem:push_up}
	Consider we do a push up operation from the weak-complete subtree $T$ of height $h_2$ to a weak-complete brother subtree $S$ of height $h_1$ ($h_2 > h_1$ where $h_1$ is calculated after moving the node and $h_2$ is calculated before moving the node). Assuming $|V(T)| + |V(S)| \leq \frac{n}{9k}$, the total distance decreases.  
\end{lemma}
\begin{proof}
	Let $u$ (a leaf of $T$) be the place from where the node was removed and let $v$ (a leaf of $S$) where we place the node. The total distance is affected: all the terms with $u$, i.e., $d_G(u, x)$ terms, are removed and $n - 1$ new terms $d_G(v, x)$ with $v$ are added.
	
	Let us denote the path from the root of $T$ to $u$ with $t_1, t_2, \ldots, t_{h_2 + 1}$ with $t_1$ being the root and $t_{h_2 + 1}$ being $u$. Let us also denote the subtree formed by $t_i$ and its child trees other than the one with $u$. %starting with $t_{i+1}$ with $T_i$.
	The same notation we use for the tree $S$ and the node $v$. You can see the tree at Figure~\ref{fig:pushup}.
	
	We define $R := G \setminus (S \cup T)$.
	
	\begin{figure}[H]
		\centering
		\includegraphics[scale=0.4]{pictures/push_up.png}
		\caption{Push up Lemma notation}
		\label{fig:pushup}
	\end{figure}
	
	Our goal now is to calculate the difference in the total distance after the push up operation. This difference consists of three parts:
	\begin{enumerate}
		\item %$v$ is closer than $u$ to all the nodes in $S$.
		We denote the change in distance for nodes in $S$ ($v$ is closer to them than $u$):
		\begin{align*}
			\Delta_1 := \sum\limits_{w \in V(S)}d_{G}(u, w) - \sum\limits_{w \in V(S)}d_{G}(v, w)
		\end{align*} 
		\item %$v$ is further than $u$ from some nodes in $T$.
		We denote the change in distance for nodes in $T$ ($u$ is closer to some nodes than $v$):
		\begin{align*}
			\Delta_2 := \sum\limits_{w \in V(T)}d_{G}(v, w) - \sum\limits_{w \in V(T)}d_{G}(u, w)
		\end{align*} 
		\item %$v$ is closer than $u$ to all the nodes in $R$.
		We denote the change in distance for nodes in $R$ ($v$ is closer to them than $u$):
		\begin{align*}
			\Delta_3 := \sum\limits_{w \in V(R)}d_{G}(u, w) - \sum\limits_{w \in V(R)}d_{G}(v, w)
		\end{align*} 
	\end{enumerate}
	
	hence the total distance is changed by $\Delta := \Delta_2 - \Delta_1 - \Delta_3$. We want to prove that $\Delta$ is negative, thus, the total distance decreases.
	
	We can lower bound $\Delta_3$ easily: 
	\begin{align*} 
		\Delta_3 = (h_2 - h_1) \cdot |V(R)| \Rightarrow\\
		\Delta_3 \geq (h_2 - h_1)\cdot (9k -1)(|V(T)| + |V(S)|) > 8k|V(T)|\\
	\end{align*} 
	
	Let us now find an upper bound for $\Delta_2$.
	
	At first, we define the Total Distance to Root (or TDR) function for tree $W$ rooted at $r$ as 
	\begin{align*}
		TDR(W) = \sum\limits_{v \in V(W)}d_{W}(v, r)
	\end{align*} 
	We say that $T_i$ is rooted at $t_i$.
	
	So the total distance from $u$ and $v$ to the nodes of $T$ can be expressed in terms of this function
	\begin{align*}
		\sum\limits_{w \in V(T)}d_{G}(v, w) = \sum\limits_{i = 1}^{h_2}\left(|V(T_i)| \cdot (h_1 + i + 1) + TDR(T_i)\right)\\
		\sum\limits_{w \in V(T)}d_{G}(u, w) = \sum\limits_{i = 1}^{h_2}\left(|V(T_i)| \cdot (h_2 - i + 1) + TDR(T_i)\right)
	\end{align*}
	
	The intuition behind those formulas is that in order to travel from $v$ to all the nodes in $T_i$ we first need to travel to its root $t_i$ which is at the distance $(h_1 + i + 1)$. We do it for each node, so $|V(T_i)|$ times. And then we travel from the root to node, accumulating $TDR(T_i)$ in total. The same for $u$ but the distance to $t_i$ decreases. 
	
	Thus,
	\begin{align*}
		\Delta_2 &= \sum\limits_{i = 1}^{h_2}|V(T_i)|(2i + h_1 - h_2)\\
		&=-(2(h_2 - 1) + h_1 - h_2) +  \sum\limits_{i = 1}^{h_2 + 1}|V(T_i)|(2i + h_1 - h_2)\\
		&= -(h_2 + h_1 - 2) + (h_1- h_2)\sum\limits_{i=1}^{h_2 + 1}|V(T_i)| + 2\sum\limits_{i =1}^{h_2 + 1}i\cdot |V(T_i)|\\
		&= -(h_2 + h_1 - 2) + |V(T)|(h_1 - h_2) + 2\sum\limits_{i =1}^{h_2 + 1}i\cdot |V(T_i)|\\
		& \leq 1 - |V(T)| + 2\sum\limits_{i =1}^{h_2 + 1}i\cdot |V(T_i)|\\
		&\leq 2\sum\limits_{i =1}^{h_2 + 1}i\cdot |V(T_i)|
	\end{align*}
	
	Each $T_i$ consists of root $t_i$ and $k -1$ weak-complete $k$-ary trees of height $\leq h_2 - i$. Therefore,
	
	\begin{align*}
		|V(T_i)| &\leq 1 + (k - 1) \cdot (1 + k + k^2 + \ldots + k^{h_2 - i})\\
		&= 1 + (k - 1) \cdot \frac{k^{h_2 - i + 1} - 1}{k - 1}\\
		&= k^{h_2 - i + 1}
	\end{align*}
	
	By that we can upper bound $\Delta_2$ further:
	\begin{claim}
		\label{clm:push_up}
		$\Delta_2 \leq 8k|V(T)|$
	\end{claim}
	\begin{proof}
		\begin{align*}
			\Delta_2 &\leq 2k^{h_2 + 1}\sum\limits_{i =1}^{h_2 + 1}\frac{i}{k^i}\\
			&\leq  2k^{h_2 + 1}\frac{k}{(k-1)^2}\\
	 		&= 2\frac{k^{h_2 + 1} - 1}{k - 1} \cdot \frac{k}{k - 1} + \frac{2k}{(k-1)^2}\\
	 		&\leq \frac{2k}{k - 1}k|V(T)| + 4\\
	 		&\leq 8k|V(T)|
		\end{align*}
	\end{proof}
	
	Recall that $\Delta_3 > 8k|V(T)|$ and $\Delta_1 \geq 0$. So we obtain that $\Delta < 0$.
\end{proof}

\begin{corollary}
	\label{cor:push_up1}
	For each subtree $S$ of an optimal tree $T$ if $|V(S)| \leq \frac{|V(T)|}{9k}$ then $S$ is a weak-complete tree.
\end{corollary}
\begin{proof}
	We prove this statement using the induction on the height of $S$.
	
	At first, we prove the base. If $S$ is of height 2, then all of its subtrees are either empty or of height 1 or 0 and, thus, they are weak-complete. Suppose that $S$ is not weak-complete. Thus, we deduce that there is a subtree of height 1 and an empty subtree, so we can perform a push up operation improving the total distance which contradicts the optimality of $T$.
	
	So now we may assume that by the inductive hypothesis all the subtrees of $S$ are weak-complete.
	
	Suppose that $S$ is not weak-complete. However, all of its subtrees are weak-complete trees, thus, there are two subtrees of $S$ such that we can perform a push up operation between them decreasing the total cost, which contradicts the optimality of $T$.
\end{proof}

\begin{corollary}
	\label{cor:push_up2}
	Consider we do a push up operation from the weak-complete subtree $T$ of height $h_2$ to a weak-complete brother subtree $S$ of height $h_1$ ($h_2 > h_1$ where $h_1$ is calculated after moving the node and $h_2$ is calculated before moving the node). The total distance increases by $O(kn)$.
\end{corollary}
\begin{proof}
	Using the notation of Lemma \ref{lem:push_up}, the total distance increases by at most $\Delta_2$ which according to Claim \ref{clm:push_up} is $\leq 8k|V(T)| = O(kn)$
\end{proof}

==> statements/subcentroid_lemma.tex <==
\begin{lemma}
	\label{lem:subcentroid}
	If we root an optimal tree $T$ at its centroid, then for each subtree $S$ its centroid is either a root of $S$ or a child of a root.
\end{lemma}
\begin{proof}
	Denote the root of $S$ as $r$.
	
	If all subtrees of $r$ have size $\leq \frac{|V(S)|}{2}$, then $r$ is a centroid of $T$ and the statement holds.
	
	Denote the subtrees of $r$ as $S_{1}, \ldots, S_{k}$.
	
	If $r$ is not a centroid, one of the $S_{j}$ is bigger than $\frac{|V(S)|}{2}$. W.l.o.g., it is $S_{1}$. We now prove that the root of $S_{1}$ is a centroid of $S$.
	
	Denote the root of $S_{1}$ as $r_{1}$ and its subtrees as $S_{11}, \ldots, S_{1k}$.
	
	Assume $r_{1}$ is not a centroid. Then it means that either $\left(\bigcup\limits_{i \in [2, \ldots, k]} S_{i} \right) \cup r$ is bigger than $\frac{|V(S)|}{2}$ or $S_{1j}$  is bigger than $\frac{|V(S)|}{2}$ for some $j \in [1,\ldots,k]$.
	
	\va{We need some picture here. Or at list reference to Figure 5.}
	
	\begin{itemize}
		\item Suppose that $\bigcup\limits_{i \in [2, \ldots, k]} S_{i} \cup r$ is bigger than $\frac{|V(S)|}{2}$. %for some $j \in [2,\ldots,k]$
		This is impossible since we already know that $|V(S_{1})| > \frac{|V(S)|}{2}$.
		
		\item $S_{1i}$  is bigger than $\frac{|V(S)|}{2}$ for some $i \in [1,\ldots,k]$. W.l.o.g., this tree is $S_{11}$.
		
		But then we can swap $S_{11}$ with any of $S_{i}$, say $S_{2}$ to be certain, to decrease the total cost. Now, we prove it.
		
		We refer to the total cost expressed in terms of edge potentials. Note that the potential changes only for $(r_{1}, r)$ edge. \va{sounds strange. $r-r_{2}$ and $r_{11}-r_{1}$ seems to change also. but they changed their potentials, so the sum is still the same.}
		
		The old value for its potential is
		\begin{align*}
			(1 + |V(S_{11})| + \sum\limits_{i = 2}^k |V(S_{1i})|) \cdot (|V(R)| + |V(S_{2})| + \sum\limits_{i = 3}^k|V(S_{j})|)
		\end{align*}
		
		while the new one is 
		\begin{align*}
			(1 + |V(S_{2})| + \sum\limits_{i = 2}^k |V(S_{1i})|) \cdot (|V(R)| + |V(S_{11})| + \sum\limits_{i = 3}^k|V(S_{i})|).
		\end{align*}
		
		Thus, the difference between the old and the new potentials is
		\begin{align*}
			(|V(S_{11})| - |V(S_{2})|)\cdot (|V(R)| + \sum\limits_{i = 3}^k|V(S_{i})| - \sum\limits_{i = 2}^k |V(S_{1i})| - 1)
		\end{align*}
		
		which is $> 0$ since $|V(S_{11})| > |V(S_{2})|$ and $|V(R)|$ is bigger than the half of the tree, in other words,
		\begin{align*}
			|V(R)| \geq \frac{n}{2} > \sum\limits_{i = 2}^k |V(S_{1i})| + 1
		\end{align*}
	\end{itemize}
	
	\begin{figure}[H]
		\centering
		\includegraphics[scale=0.5]{pictures/subcentroid_proof.png}
		\caption{Notation for Lemma \ref{lem:subcentroid}}
	\end{figure} 
\end{proof}

So we can only have two possibilities for the inner structure of each subtree of an optimal tree (rooted at its centroid).

\begin{figure}[H]
	\centering
	\begin{minipage}[b]{0.35\textwidth}
		\includegraphics[width=\textwidth]{pictures/local_decomposition_v1.png}
		\caption{Case 1}
		\label{fig:local_decomposition_v1}
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.6\textwidth}
		\includegraphics[width=\textwidth]{pictures/local_decomposition_v2.png}
		\caption{Case 2}
		\label{fig:local_decomposition_v2}
	\end{minipage}
\end{figure}

\begin{corollary}
	\label{cor:subcentroid}
	If we root an optimal tree $T$ at its centroid, then for each subtree $S$ at level $2h,\ h \in \mathbb{N}_0$ $|V(S)| \leq \frac{|V(T)|}{2^h}$
\end{corollary}
\begin{proof}
	We prove by induction.
	
	The statement holds for $h = 0$.
	
	Consider a subtree $Q$ at level $2(h + 1)$ and a tree $P$ rooted at a grandparent of a root of $Q$. By Lemma \ref{lem:subcentroid} $|V(Q)| \leq \frac{|V(P)|}{2}$ which by induction hypothesis $\leq \frac{|V(T)|}{2^h \cdot 2} = \frac{|V(T)|}{2^{h + 1}}$
\end{proof}

==> statements/uniform_potential.tex <==
\begin{observation}
In a uniform workload a potential from Definition~\ref{def:edge_potential} of an edge connecting two subtrees $S$ and $T$ is equal to $|V(S)| \cdot |V(T)|$. 
\end{observation}

==> statements/w_uniform_claim.tex <==
\begin{claim}
    \label{clm:w uniform}
    In the uniform workload scenario, $W[i, i - 1 + l] = W[j, j - 1 + l]$ for any $l \in [1, n]$ and any $i,j \in [1, n - l]$. In other words, $W$ of the segment depends only on its length, not position. 
    
    Moreover, $W[i, j]$ can be computed in $O(1)$.
\end{claim}
\begin{proof}
    Recall that intuitively $W[i, j]$ indicates the number of requests going out of the segment $[i, j]$. Since each node within the segment communicates exactly once with each node outside the segment
    \begin{align*}
        W[i, i - 1 + l] = l (n - l)
    \end{align*}
\end{proof}
